Variational Inference for Graph Convolutional Networks in the Absence of Graph Data and Adversarial Settings

We propose a framework that lifts the capabilities of graph convolutional networks (GCNs) to scenarios where no input graph is given and increases their robustness to adversarial attacks. We formulate a joint probabilistic model that considers a prior distribution over graphs along with a GCN-based likelihood and develop a stochastic variational inference algorithm to estimate the graph posterior and the GCN parameters jointly. To address the problem of propagating gradients through latent variables drawn from discrete distributions, we use their continuous relaxations known as Concrete distributions. We show that, on real datasets, our approach can outperform state-of-the-art Bayesian and non-Bayesian graph neural network algorithms on the task of semi-supervised classification in the absence of graph data and when the network structure is subjected to adversarial perturbations.

==> changes_for_final_CMT_form.tex <==
Please explain how you have modified your paper to address reviewer and area chair feedback.

(1) Qualitative analysis: We have added an analysis of the learned graphs in sec. 4.4 and Fig. 4 in the main paper and provided additional examples in the supplement (sec. M).

(2) Consistency of prior work and introduction: We have explicitly acknowledged prior work addressing the same types of problems (along with their references) in the introduction (p. 2, second paragraph) so as to make it more consistent with sec. 1.1. 

(3) Prior knowledge on LDS: We have expanded on our explanation of the difficulties of incorporating prior knowledge in LDS [13] in sec. 1.1.

(4) Relation to neural relational inference: We have provided a reference to [23] and a description of its relation to our work in sec 1.1 (bottom paragraph).

(5) Reducing the number of parameters: With experiments on the PubMed dataset, we have provided in the supplement (sec. O) an example of how our approach can be combined with other techniques such as cluster GCN  so as to reduce the number of parameters and allow for mini-batch training. We have referenced this in sec. 3.4 in the main paper. 

(6) Influence of the KL term in training: We have analyzed this in sec. K of the supplement.



==> context_and_details_icml_resubmission.tex <==
% This has what was submitted to CMT re ICML rejection
A previous version of this work was submitted to ICML 2020. Below we describe our major changes to the submission as a response to ICML reviewers’ feedback that suggested a comparison with robust GCN (RGCN; Zhu et al, KDD, 2019) in the adversarial setting and evaluation of our method on the ground truth (uncorrupted) graphs were necessary.

Comparison with robust GCN (RGCN; Zhu et al, KDD, 2019): We now provide a comparison with RGCN in the adversarial setting (section 4.2). The results show that our approach outperforms consistently RGCN on the citation networks and is on par or better than this method on PolBlogs.

Performance on ground truth graphs: We now present results on the ground truth graphs for the datasets considered in section 4.2. We are pleased to report that, even when using the noise-free graphs associated with the original datasets and believed to be most beneficial, the results show that our method outperforms all the other competing baselines, including the original GCN framework. This shows that our approach managed to discover better graph structures that improve the performance on the given semi-supervised classification problem. 

Other concerns: We have also modified the text incorporating some of the reviewers’ comments, clarifying and expanding on our contribution  (in the abstract and in the introduction) and differences with previous work in sections 1.1 and 4. 



==> hierarchical.tex <==
\section{Hierarchical Approach}
\newcommand{\prior}{\berndiscreteprior}
\newcommand{\allprior}{\alldiscreteprior}
Here we consider a hierarchical approach in the discrete case. Let us define the following joint distribution:
\begin{align}
    p(\alldiscreteprior, \mbA, \Yobs \g \mbX, \mbtheta,\mbalpha, \mbbeta) &= p(\alldiscreteprior \g \mbalpha, \mbbeta) p(\mbA \g \alldiscreteprior) p_\mbtheta(\Yobs \g \mbA, \mbX ), \text{ where} \\
     p(\alldiscreteprior \g \mbalpha, \mbbeta) &= \prod_{ij} \Beta(\berndiscreteprior_{ij}; \alpha_{ij}, \beta_{ij}), \\
     p(\mbA \g \alldiscreteprior) &= \prod_{ij} \Bern(A_{ij}; \berndiscreteprior_{ij}),\\
     p_\mbtheta(\Yobs \g \mbA, \mbX ) &= \prod_{\mby_n \in \Yobs} p_{\mbtheta}(\mby_n \g \mbX, \mbA).
\end{align}
Now we define the joint variational $q(\alldiscreteprior, \mbA) = q(\alldiscreteprior) q(\mbA) $:
\begin{align}
    q(\mbA \g \mbphi) &= \prod_{ij} \Bern(A_{ij}; \phi_{ij}) \\
    q(\alldiscreteprior | \tilde{\mbalpha}, \tilde{\mbbeta}) &= \prod_{ij} \Beta(\berndiscreteprior_{ij}; \tilde{\alpha}_{ij}, \tilde{\beta}_{ij}).
\end{align}
Hence the variational lower bound  is given by
\begin{equation}
\begin{split}
    \elbo  & =\E_q(\mbA, \allprior) \left[ \log \frac{ p(\alldiscreteprior, \mbA, \Yobs \g \mbX, \mbtheta,\mbalpha, \mbbeta)}{q(\mbA, \allprior)} \right]  \\
     & =  \E_q \left[\log p(\alldiscreteprior \g \mbalpha, \mbbeta)  \right]
     + \E_q \left[ \log p(\mbA \g \alldiscreteprior)  \right] 
     + \E_q \left[ \log  p_\mbtheta(\Yobs \g \mbA, \mbX ) \right] \\
    & \quad - \E_q  \left[ \log q(\allprior) \right] 
     - \E_q  \left[ \log q(\mbA) \right].
\end{split}
\end{equation}
Let $\psi(x) \equiv \frac{d}{dx} \log \Gamma(x)$ be the digamma function. Hence
For each of the terms above we have
\begin{equation}
\begin{split}
    \E_q \left[\log p(\alldiscreteprior \g \mbalpha, \mbbeta)  \right] 
    &= \sum_{ij} \log \Gamma(\alpha_{ij} + \beta_{ij})  - \log \Gamma(\alpha_{ij}) - \log \Gamma(\beta_{ij}) \\
    & + (\alpha_{ij} - 1) \left[ \psi(\tilde{\alpha}_{ij}) - \psi(\tilde{\alpha}_{ij} + \tilde{\beta}_{ij}) \right]\\
    & + (\beta_{ij} -1) \left[ \psi(\tilde{\beta_{ij}}) - \psi(\tilde{\alpha_{ij}} + \tilde{\beta}_{ij})\right].
\end{split}
\end{equation}

\begin{equation}
    \E_q \left[ \log p(\mbA \g \alldiscreteprior)  \right] 
    = \sum_{ij} \phi_{ij} \left[ \psi(\tilde{\alpha}_{ij}) - \psi(\tilde{\alpha}_{ij} + \tilde{\beta}_{ij} )\right]
    + (1 - \phi_{ij}) \left[ \psi(\tilde{\beta}_{ij}) - \psi(\tilde{\alpha}_{ij} + \tilde{\beta}_{ij}) \right].
\end{equation}

\begin{equation}
    \begin{split}
        - \E_q  \log q(\allprior) 
         &= \sum_{ij} - \log \Gamma(\tilde{\alpha}_{ij} + \tilde{\beta}_{ij})
         + \log \Gamma(\tilde{\alpha}_{ij}) + \log \Gamma(\tilde{\beta}_{ij}) \\
         & \quad - (\tilde{\alpha}_{ij} -1) \left[ \psi(\tilde{\alpha}_{ij}) - \psi(\tilde{\alpha}_{ij} + \tilde{\beta}_{ij}) \right] \\
         & \quad - (\tilde{\beta}_{ij} -1) \left[ \psi(\tilde{\beta}_{ij}) - \psi(\tilde{\alpha}_{ij} + \tilde{\beta}_{ij}) \right] 
    \end{split}
\end{equation}

\begin{equation}
     - \E_q  \log q(\mbA)  
     = -  \sum_{ij} \left[ \phi_{ij} \log \phi_{ij} + (1 - \phi_{ij}) \log (1 - \phi_{ij}) \right]
\end{equation}
The only term left is the \gls{ELL}  $\E_q \left[ \log  p_\mbtheta(\Yobs \g \mbA, \mbX ) \right]$, which can be estimated using \gls{MC} sampling. 

==> supp_experiments.tex <==
\section{Additional results}

\subsection{Smooth parameterization}
\label{sec:smooth}
\Cref{fig:smooth-param} compares a typical run of our algorithms using the free and smooth parameterizations of the posterior. We see that the optimizer struggles to find directions of improvement for the free parameterization, whereas for the smooth parameterization the \gls{NELBO} decreases steadily during optimization. This behavior was observed throughout several learning rate settings and we attribute it to the discrete combinatorial optimization nature of the \gls{NELBO} when using the free parameterization.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{../figures/elbo_comparison}
	\caption{The \acrfull{NELBO} as a function of the number of epochs for the freely parameterized posterior (Free) and the smooth parameterization (Lowrank).
	\label{fig:smooth-param}}
\end{figure}

\subsection{Noiseless graphs}
\Cref{tab:noiseless-graphs} shows the results for the noisy graphs where we see that our approach performs similarly to standard \glspl{GCN}.
\input{table_noiseless_results}

\subsection{Noisy graphs}
\label{sec:supp-noisy}
Test \acrfull{MLL} results are given in \cref{fig:noisy-graphs-relaxed-mll}. 
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{../figures/citeseer_relaxed_adding_mean_test_likelihood}
\includegraphics[width=0.45\textwidth]{../figures/cora_relaxed_adding_mean_test_likelihood}
\caption{Results for noisy graphs on \citeseer (left) and \cora (right): \Acrfull{MLL} as a function of the ratio of additional fake links relative to the number of true links. 
	\acrshort{BGCNR}-$\smoothfactorone$ stands for the relaxed version of our method with smoothing factor $\smoothfactorone$.   		
	\label{fig:noisy-graphs-relaxed-mll} }
\end{figure}

 

\subsection{Feature-based graphs}
Following the methods of \cite{henaff2015deep}, a graph was estimated using \cora and \citeseer based on the node features. Given a training set with features and labels we train a fully connected network with $1$-hidden layer, $Q\in \{16,32\}$ neurons using standard \gls{RELU} activation and $0.5$ dropout between each layer. We then extract the first layer features $\tilde{\mbZ}_1 \in \mathbb{R}^{M \times Q}$ where $M$ includes training, validation and test sets and consider their distance, $d(i,j) = \parallel \tilde{\mbZ}_{1,i}-\tilde{\mbZ}_{1,j}\parallel^2$. The adjacency matrix, $\mbA$, was constructed by taking the $K\in\{8,16,32\}$ closest neighbors. Test \acrfull{MLL} results are given in \cref{fig:feature-graphs-relaxed-mll}. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{../figures/citeseer_supervised_graph_meantestlikelihood}
	\includegraphics[width=0.45\textwidth]{../figures/cora_supervised_graph_mean_test_likelihood}
	\caption{Results for feature-based graphs on \citeseer (left) and \cora (right): \Acrfull{MLL} as a function of $Q$-$K$ settings, where $Q$ is the number of hidden units and $K$ the number of neighbors used to construct the graph.  
		\acrshort{BGCNR}-$\smoothfactorone$ stands for the relaxed version of our method with smoothing factor $\smoothfactorone$. 
		\label{fig:feature-graphs-relaxed-mll}}
\end{figure}



\input{twitter}





%\subsection{Discrete posterior}
%Include all the results for the discrete posterior here


==> supp_title.tex <==
% For affiliations
\newcommand{\footremember}[2]{%
	\thanks{#2}
	\newcounter{#1}
	\setcounter{#1}{\value{footnote}}%
}
\newcommand{\footrecall}[1]{%
	\footnotemark[\value{#1}]%
}

\title{Variational Inference for Graph Convolutional Networks in the Absence  of Graph Data and Adversarial Settings:\\ \emph{Supplementary Material}}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\author{
Pantelis Elinas\footremember{joint}{Joint first author.}\\
\texttt{pantelis.elinas@data61.csiro.au} \\
CSIRO's Data61
\And
Edwin V.~Bonilla\footrecall{joint}\\
\texttt{edwin.bonilla@data61.csiro.au} \\
CSIRO's Data61 and The University of Sydney
\And
Louis Tiao\\
\texttt{louis.tiao@sydney.edu.au} \\
The University of Sydney and CSIRO's Data61\\
}

%\author{%
%  Pantelis Elinas \\
%  CSIRO's Data61\\
%  \texttt{hippo@cs.cranberry-lemon.edu} \\
%  % examples of more authors
%  % \And
%  % Coauthor \\
%  % Affiliation \\
%  % Address \\
%  % \texttt{email} \\
%  % \AND
%  % Coauthor \\
%  % Affiliation \\
%  % Address \\
%  % \texttt{email} \\
%  % \And
%  % Coauthor \\
%  % Affiliation \\
%  % Address \\
%  % \texttt{email} \\
%  % \And
%  % Coauthor \\
%  % Affiliation \\
%  % Address \\
%  % \texttt{email} \\
%}
\maketitle

